Anchor-based Large Language Models

Large language models (LLMs) predominantly employ decoder-only transformer architectures, necessitating the retention of keys/values information for historical tokens to provide contextual information and avoid redundant computation. However, the substantial size and parameter volume of these LLMs require massive GPU memory. This memory demand increases with the length of the input text, leading to an urgent need for more efficient methods of information storage and processing. This study introduces Anchor-based LLMs (AnLLMs), which utilize an innovative anchor-based self-attention network (AnSAN) and also an anchor-based inference strategy. This approach enables LLMs to compress sequence information into an anchor token, reducing the keys/values cache and enhancing inference efficiency. Experiments on question-answering benchmarks reveal that AnLLMs maintain similar accuracy levels while achieving up to 99% keys/values cache reduction and up to 3.5 times faster inference. Despite a minor compromise in accuracy, the substantial enhancements of AnLLMs employing the AnSAN technique in resource utilization and computational efficiency underscore their potential for practical LLM applications.

==> latex/backgrounds.tex <==
\section{Background of Self-Attention Networks}

introduce the principle of san;

then the key/value cache during inference

==> tables/main_mmlucsqa.tex <==

\begin{table*}[t]

\centering

\begin{subtable}[h]{1.0\textwidth}
\centering
\begin{tabular}{lcccccccccc}
\toprule
 & & \bf BoolQ & \bf PIQA & \bf SCIQ & \bf HS & \bf WG & \bf ARC-e & \bf ARC-c & 
 \bf OBQA & \bf AVG.  \\ \midrule

 \multirow{2}{*}{\bf Llama2} & 7B & 77.7 & 78.1 & 93.7 & 57.1 & 69.1 & 76.3 & 43.4 & 31.4 & 65.8 \\
     & 13B & 80.6  & 79.1 & 94.5 & 60.0 & 72.1 & 79.4 & 48.5 & 35.2 & 68.7 \\  \midrule

 \multirow{2}{*}{\bf ALLM-ADDT} & 7B &  \\
      & 13B &  \\ \cdashline{1-11}[2.5pt/5pt]\noalign{\vskip 0.5ex} 

 \multirow{2}{*}{\bf \quad w/o ASAN} & 7B &  \\
                         & 13B &2&3&4&5&6&7&8&9 \\ \midrule

 
 \multirow{2}{*}{\bf ALLM-PUNC} & 7B & 68.4 & 74.5 & 86.4 & 48.2 & 65.0 & 70.1 & 38.8 & 30.2 & 60.2 \\
 & 13B & 72.6 & 78.0 & 89.3 & 54.7 & 68.8 & 77.1 & 43.9 & 36.4 & 65.1 \\ \cdashline{1-11}[2.5pt/5pt]\noalign{\vskip 0.5ex} 

 \multirow{2}{*}{\bf \quad w/o ASAN} & 7B & 74.5 & 77.9 & 93.1 & 55.4 & 67.4 & 73.8 & 41.4 & 30.6 & 64.3 \\
      & 13B & 75.4 & 78.8 & 93.9 & 58.3 & 71.3 & 78.5 & 46.6 & 37.0 &67.5  \\


    
\bottomrule
\end{tabular}
\caption{Performance on Standard Benchmark.}
\label{tab:avgsenteval}

\end{subtable}

\begin{subtable}[h]{1.0\textwidth}
\centering
\begin{tabular}{lccccccccc}
\toprule
 & & BoolQ & PIQA & SCIQ & HS & WG & ARC-e & ARC-c & OBQA  \\ \midrule

 \multirow{2}{*}{Text} & $L_{Demo}$ &2&3&4&5&6&7&8&9 \\
                         & $L_{x}$ &2&3&4&5&6&7&8&9 \\  \midrule


   Llama2   & KV &2&3&4&5&6&7&8&9 \\ \midrule


 ALLM-ADDT & KV &2&3&4&5&6&7&8&9 \\ \cdashline{1-10}[2.5pt/5pt]\noalign{\vskip 0.5ex} 

 ALLM-PUNC & KV &2&3&4&5&6&7&8&9 \\

    
\bottomrule
\end{tabular}
\caption{Text lengths and Key/Value Cache.}
\label{tab:avgsenteval}

\end{subtable}

\begin{subtable}[h]{1.0\textwidth}
\centering
\begin{tabular}{lccccccccc}
\toprule
 & & BoolQ & PIQA & SCIQ & HS & WG & ARC-e & ARC-c & OBQA  \\ \midrule

 % \multirow{2}{*}{Llama2} & 7B &2&3&4&5&6&7&8&9 \\
 %                         & 13B &2&3&4&5&6&7&8&9 \\  \midrule

 \multirow{2}{*}{ALLM-ADDT} & 7B &2&3&4&5&6&7&8&9 \\
  & 13B &2&3&4&5&6&7&8&9 \\ \cdashline{1-10}[2.5pt/5pt]\noalign{\vskip 0.5ex} 

 \multirow{2}{*}{ALLM-PUNC} & 7B &2&3&4&5&6&7&8&9 \\
                         & 13B &2&3&4&5&6&7&8&9 \\

    
\bottomrule
\end{tabular}
\caption{Inference acceleration ratios.}
\label{tab:avgsenteval}

\end{subtable}

\caption{Classification accuracy on SentEval probing tasks of evaluating the linguistic properties. "+BT" means training a translation model with BT synthetic parallel data. "MLM+CLM+DAE" means the joint objective of the three self-supervised objectives.} 
\label{tab:probingtaskacc}

\end{table*}

==> tables/main_mmlucsqa_2.tex <==

\begin{table*}[t]

\centering

\begin{subtable}[h]{1.0\textwidth}
\centering
\begin{tabular}{lccccccccc}
\toprule
 &  \bf BoolQ & \bf PIQA & \bf SCIQ & \bf HS & \bf WG & \bf ARC-e & \bf ARC-c & 
 \bf OBQA & \bf AVG.  \\ \midrule

\bf Llama2-7B & 77.7 & 78.1 & 93.7 & 57.1 & 69.1 & 76.3 & 43.4 & 31.4 & 65.8 \\ \cdashline{1-10}[2.5pt/5pt]\noalign{\vskip 0.5ex} 
 \quad +ASAN &  65.0 & 71.9 & 83.0 & 43.3 & 66.5 & 71.0 & 38.6 & 30.0 & 58.7 \\ \midrule

\bf ALLM-AC &  77.0 & 78.3 & 93.8 & 54.7 & 68.5 & 74.4 & 42.5 & 31.6 & 65.1 \\ \cdashline{1-10}[2.5pt/5pt]\noalign{\vskip 0.5ex} 
 \quad +ASAN &  \\ \midrule

\bf ALLM-PC & 74.4 & 77.8 & 94.4 & 55.0 & 68.0 & 73.4 & 40.8 & 33.2 & 64.6  \\ \cdashline{1-10}[2.5pt/5pt]\noalign{\vskip 0.5ex} 
\quad+ASAN &  72.1 & 77.5 & 90.7 & 52.2 & 65.9 & 72.4 & 39.1 & 33.6 & 62.9 \\ 
    
\bottomrule
\end{tabular}
\caption{0-shot Performance on Standard Benchmark.}
\label{tab:avgsenteval}

\end{subtable}

\begin{subtable}[h]{1.0\textwidth}
\centering
\begin{tabular}{lcccccccccc}
\toprule
 & & \bf BoolQ & \bf PIQA & \bf SCIQ & \bf HS & \bf WG & \bf ARC-e & \bf ARC-c & 
 \bf OBQA & \bf AVG.  \\ \midrule

 & $L_{demo}$ &  \\ 
  & $L_{x}$ &  \\  \midrule

\bf Llama2-7B & \emph{Acc} & 78.4 & 78.7 & 96.8 & 58.3 & 73.7 & 79.8 & 50.0 & 37.2 & 69.1 \\ 
           & $L_{kv}$ \\ 
           & \emph{T(s)} \\  \cdashline{1-11}[2.5pt/5pt]\noalign{\vskip 0.5ex} 
 \quad +ASAN &  \emph{Acc} & 50.8 & 68.3 & 65.7 & 30.8 & 68.6 & 62.6 & 35.8 & 34.6 & 52.1 \\ 
           & $L_{kv}$ \\ 
           & \emph{T(s)} \\ \midrule

\bf ALLM-AC & \emph{Acc} &  \\ 
           & $L_{kv}$  \\ 
           & \emph{T(s)} \\  \cdashline{1-11}[2.5pt/5pt]\noalign{\vskip 0.5ex} 
 \quad +ASAN &   \emph{Acc} & 76.6 & 78.7 & 95.7 & 55.6 & 70.6 & 79.2 & 47.9 & 35.6 & 67.5 \\ 
           & $L_{kv}$ & 5 & 5 & 5 & 5 & 5 & 5 & 5 & 5 & 5 \\ 
           & \emph{T(s)} \\ \midrule


\bf ALLM-PC & \emph{Acc} & 74.0 & 78.1 & 96.6 & 55.3 & 71.0 & 79.4 & 49.4 & 36.8 & 67.6 \\ 
           & $L_{kv}$ \\ 
           & \emph{T(s)} \\  \cdashline{1-11}[2.5pt/5pt]\noalign{\vskip 0.5ex} 
 \quad +ASAN & \emph{Acc} & 73.4 & 78.2 & 93.1 & 52.6 & 68.0 & 76.7 & 45.6 & 36.2 & 65.5 \\ 
           & $L_{kv}$ \\ 
           & \emph{T(s)} \\ \midrule





    
\bottomrule
\end{tabular}
\caption{5-shot Performance on Standard Benchmark.}
\label{tab:avgsenteval}

\end{subtable}


\caption{Classification accuracy on SentEval probing tasks of evaluating the linguistic properties. "+BT" means training a translation model with BT synthetic parallel data. "MLM+CLM+DAE" means the joint objective of the three self-supervised objectives.} 
\label{tab:probingtaskacc}

\end{table*}

==> tables/main_mmlucsqa_3.tex <==

\begin{table*}[t]

\centering

\begin{subtable}[h]{1.0\textwidth}
\centering
\begin{tabular}{lccccccccc}
\toprule
 &  \bf BoolQ & \bf PIQA & \bf SCIQ & \bf HS & \bf WG & \bf ARC-e & \bf ARC-c & 
 \bf OBQA & \bf AVG.  \\ \midrule

\bf Llama2-7B & 77.7 & 78.1 & 93.7 & 57.1 & 69.1 & 76.3 & 43.4 & 31.4 & 65.8 \\ 
% \cdashline{1-10}[2.5pt/5pt]\noalign{\vskip 0.5ex} 
 % \quad +ASAN &  65.0 & 71.9 & 83.0 & 43.3 & 66.5 & 71.0 & 38.6 & 30.0 & 58.7 \\ \midrule
% \cdashline{1-10}[2.5pt/5pt]\noalign{\vskip 0.5ex} 
 % \quad +ASAN &  \\ \midrule

\bf ALLM-PC & 74.4 & 77.8 & 94.4 & 55.0 & 68.0 & 73.4 & 40.8 & 33.2 & 64.6  \\ 

\bf ALLM-AC &  77.0 & 78.3 & 93.8 & 54.7 & 68.5 & 74.4 & 42.5 & 31.6 & 65.1 \\ 
% \cdashline{1-10}[2.5pt/5pt]\noalign{\vskip 0.5ex} 
% \quad+ASAN &  72.1 & 77.5 & 90.7 & 52.2 & 65.9 & 72.4 & 39.1 & 33.6 & 62.9 \\ 
    
\bottomrule
\end{tabular}
\caption{0-shot Performance on Standard Benchmark.}
\label{tab:avgsenteval}

\end{subtable}

\begin{subtable}[h]{1.0\textwidth}
\centering
\begin{tabular}{lcccccccccc}
\toprule
 & & \bf BoolQ & \bf PIQA & \bf SCIQ & \bf HS & \bf WG & \bf ARC-e & \bf ARC-c & 
 \bf OBQA & \bf AVG.  \\ \midrule

 & $L_{demo}$ &  \\ 
  & $L_{x}$ &  \\  \midrule

\bf Llama2-7B & \emph{Acc} & 78.4 & 78.7 & 96.8 & 58.3 & 73.7 & 79.8 & 50.0 & 37.2 & 69.1 \\ 
           & $L_{kv}$ \\ 
           & \emph{T(s)} \\  \cdashline{1-11}[2.5pt/5pt]\noalign{\vskip 0.5ex} 
 \quad +ASAN &  \emph{Acc} & 50.8 & 68.3 & 65.7 & 30.8 & 68.6 & 62.6 & 35.8 & 34.6 & 52.1 \\ 
           & $L_{kv}$ \\ 
           & \emph{T(s)} \\ \midrule


\bf ALLM-PC & \emph{Acc} & 74.0 & 78.1 & 96.6 & 55.3 & 71.0 & 79.4 & 49.4 & 36.8 & 67.6 \\ 
           & $L_{kv}$ \\ 
           & \emph{T(s)} \\  \cdashline{1-11}[2.5pt/5pt]\noalign{\vskip 0.5ex} 
 \quad +ASAN & \emph{Acc} & 73.4 & 78.2 & 93.1 & 52.6 & 68.0 & 76.7 & 45.6 & 36.2 & 65.5 \\ 
           & $L_{kv}$ \\ 
           & \emph{T(s)} \\ \midrule


\bf ALLM-AC & \emph{Acc} & 73.1 & 78.6 & 96.8 & 56.9 & 72.3 & 79.8 & 49.0 & 37.2 & 67.9 \\ 
           & $L_{kv}$  \\ 
           & \emph{T(s)} \\  \cdashline{1-11}[2.5pt/5pt]\noalign{\vskip 0.5ex} 
 \quad +ASAN &   \emph{Acc} & 76.6 & 78.7 & 95.7 & 55.6 & 70.6 & 79.2 & 47.9 & 35.6 & 67.5 \\ 
           & $L_{kv}$ & 5 & 5 & 5 & 5 & 5 & 5 & 5 & 5 & 5 \\ 
           & \emph{T(s)} \\ \midrule


    
\bottomrule
\end{tabular}
\caption{5-shot Performance on Standard Benchmark.}
\label{tab:avgsenteval}

\end{subtable}


\caption{Classification accuracy on SentEval probing tasks of evaluating the linguistic properties. "+BT" means training a translation model with BT synthetic parallel data. "MLM+CLM+DAE" means the joint objective of the three self-supervised objectives.} 
\label{tab:probingtaskacc}

\end{table*}

==> tables/main_mmlucsqa_4.tex <==

\begin{table*}[t]

\centering
\begin{subtable}[h]{1.0\textwidth}
\centering
\begin{tabular}{lccccccccc}
\toprule
 &  \bf BoolQ & \bf PIQA & \bf SCIQ & \bf HS & \bf WG & \bf ARC-e & \bf ARC-c & 
 \bf OBQA & \bf AVG.  \\ \midrule

\bf Llama2-7B & 77.7 & 78.1 & 93.7 & 57.1 & 69.1 & 76.3 & 43.4 & 31.4 & 65.8 \\ 

\bf ALLM-PC & 74.4 & 77.8 & 94.4 & 55.0 & 68.0 & 73.4 & 40.8 & 33.2 & 64.6  \\ 

\bf ALLM-AC &  77.0 & 78.3 & 93.8 & 54.7 & 68.5 & 74.4 & 42.5 & 31.6 & 65.1 \\ 
    
\bottomrule
\end{tabular}
\caption{The 0-shot Performance.}
\label{tab:avgsenteval}

\end{subtable}

\begin{subtable}[h]{1.0\textwidth}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccccccc}
\toprule
 & & \bf BoolQ & \bf PIQA & \bf SCIQ & \bf HS & \bf WG & \bf ARC-e & \bf ARC-c & 
 \bf OBQA & \bf AVG.  \\ \midrule

 & $L_{d}$ & 804 & 262 & 603 & 426 &	133 & 145 & 209 & 89 & 334 \\ 
  & $L_{x}$ & 169 & 42 & 130 & 90 & 26 & 36 & 42 & 18 & 69 \\  \midrule

\bf Llama2-7B & \emph{Acc} & 78.4 & 78.7 & 96.8 & 58.3 & 73.7 & 79.8 & 50.0 & 37.2 & 69.1 \\  \cdashline{1-11}[2.5pt/5pt]\noalign{\vskip 0.5ex} 
 \quad +ASAN &  \emph{Acc} & 50.8 & 68.3 & 65.7 & 30.8 & 68.6 & 62.6 & 35.8 & 34.6 & 52.1 \\   \midrule


\bf ALLM-EP & \emph{Acc} & 74.0 & 78.1 & 96.6 & 55.3 & 71.0 & 79.4 & 49.4 & 36.8 & 67.6 \\  \cdashline{1-11}[2.5pt/5pt]\noalign{\vskip 0.5ex} 
 \quad +ASAN & \emph{Acc} & 73.4 & 78.2 & 93.1 & 52.6 & 68.0 & 76.7 & 45.6 & 36.2 & 65.5 \\ 
& $L_{kv}$ & 43 & 9 & 50 & 25 & 8 & 5 & 30 & 89 & 32 \\ 
& \textcolor{forestgreen}{$\mathcal{C}_{\Downarrow}$} & \cellcolor{forestgreen!41}95\% & \cellcolor{forestgreen!49}97\% & \cellcolor{forestgreen!29}92\%  & \cellcolor{forestgreen!37}94\% & \cellcolor{forestgreen!37}94\% & \cellcolor{forestgreen!49}97\% & \cellcolor{forestgreen!5}86\% & 0\% & \cellcolor{forestgreen!21}90\% \\ \midrule


\bf ALLM-AC & \emph{Acc} & 73.1 & 78.6 & 96.8 & 56.9 & 72.3 & 79.8 & 49.0 & 37.2 & 67.9 \\  \cdashline{1-11}[2.5pt/5pt]\noalign{\vskip 0.5ex} 
 \quad +ASAN &   \emph{Acc} & 76.6 & 78.7 & 95.7 & 55.6 & 70.6 & 79.2 & 47.9 & 35.6 & 67.5 \\ 
 & $L_{kv}$ & 5 & 5 & 5 & 5 & 5 & 5 & 5 & 5 & 5 \\ 
  & \textcolor{forestgreen}{$\mathcal{C}_{\Downarrow}$} & \cellcolor{forestgreen!50}99\% & \cellcolor{forestgreen!50}98\% & \cellcolor{forestgreen!50}99\% & \cellcolor{forestgreen!50}99\% & \cellcolor{forestgreen!48}96\% & \cellcolor{forestgreen!49}97\% & \cellcolor{forestgreen!50}98\% & \cellcolor{forestgreen!37}94\% & \cellcolor{forestgreen!50} 99\% \\
    
\bottomrule
\end{tabular}
}
\caption{The 5-shot Performance.}
\label{tab:avgsenteval}

\end{subtable}


\caption{Accuracy and key/value cache in natural language understanding benchmarks. The symbol \textcolor{forestgreen}{$\mathcal{C}_{\Downarrow}$} indicates the reduction in key/value cache size during inference. \emph{Acc} stands for Accuracy. $L_{kv}$ represents the length of the key/value cache. $L_{d}$ and $L_{x}$ denote the lengths of in-context learning demonstrations and input queries, respectively.} 
\label{tab:probingtaskacc}

\end{table*}
% 请帮我将这个表格的列按照OBQA,WG, ARC-e, ARC-c,PIQA,HS,SCIQ,BoolQ的顺序重新排一下，相应的数据也跟着排序。

% \begin{itemize}[leftmargin=*,topsep=0.1em,itemsep=0.1em,parsep=0.1em]
% \item \textbf{ALLM-AC.} This strategy entails the introduction of a new token to act as the sequence anchor. In our implementation, we designate <AC> as the new token and initialize its embedding using the mean value of the embedding matrix. The function of this new token mirrors that of the [CLS] token in BERT \cite{devlin2018bert}, which is used for sequence classification tasks.

% \item \textbf{ALLM-EP.} This approach uses punctuation marks within the sequence as anchor tokens. Punctuation marks, such as commas, periods, and question marks, are viewed as semantic boundaries within a sequence. As such, they can serve as anchor tokens in ALLM. In our experiments of ALLM-EP, we use the end point in English as the anchor tokens.

% \end{itemize}

% Anchor-based Self-Attention Networks (ASAN) is to aggregate the sentence information into its anchor token respectively, thus we can discard the other tokens and reduce the keys/values caching. 
% Anchor-based Large Langauge Model (ALLM) is trained with ASAN on one-billions tokens, with Llama2-7b initialization.
% 使用ASAN虽然效果有轻微下降（1.5 accuracy左右），但是大幅度降度了keys/values caches需求。

% 这是要发到nlp的acl顶会的论文实验结果图，关于Accuracy和keys/values cache两点，帮我用地道的专业的学术英语写一份详细的分析。,突出我们的贡献。


==> tables/perplexity.tex <==
\begin{table*}[]
    \centering
\begin{tabular}{lccccccc}
\toprule
     \multirow{2}{*}{\bf Method} & \multirow{2}{*}{\bf Size}  & \multicolumn{6}{c}{\bf Evaluation Context Length} \\ \cmidrule(r){3-8}
    & & \textbf{256} & \textbf{512} & \textbf{1024} & \textbf{2048} & \textbf{4096} & \textbf{AVG.}  \\ \midrule 
    \multirow{2}{*}{\bf Llama2} & 7B  & 5.42 & 4.32 & 3.64 & 3.2  & 2.91 & 3.90   \\ 
    & 13B &  5.13 & 4.09 & 3.45 & 3.04 & 2.77 & 3.70 \\ \midrule

    \multirow{2}{*}{\bf ALLM-ADD} & 7B &   \\ 
    & 13B &   \\ \cdashline{1-8}

    \multirow{2}{*}{\bf \quad w/o ASAN} & 7B &   \\ 
    & 13B &   \\ \midrule

    \multirow{2}{*}{\bf ALLM-PUNC} & 7B &  6.76 & 5.75 & 5.23 & 4.94 & 4.8  & 5.50    \\ 
    & 13B & 6.54 & 5.33 & 4.67 & 4.28 & 4.06 & 4.98   \\ \cdashline{1-8}

    \multirow{2}{*}{\bf \quad w/o ASAN}  & 7B  & 5.65 & 4.49 & 3.79 & 3.35 & 3.06 & 4.07    \\
                & 13B & 5.63 & 4.38 & 3.66 & 3.21 & 2.93 & 3.96 \\
\bottomrule
\end{tabular}
    \caption{Caption}
    \label{tab:ppl}
\end{table*}
